Leaning-Based Control of an Immersive-Telepresence Robot

In this paper, we present an implementation of a leaning-based control of a differential drive telepresence robot and a user study in simulation, with the goal of bringing the same functionality to a real telepresence robot. The participants used a balance board to control the robot and viewed the virtual environment through a head-mounted display. The main motivation for using a balance board as the control device stems from Virtual Reality (VR) sickness; even small movements of your own body matching the motions seen on the screen decrease the sensory conflict between vision and vestibular organs, which lies at the heart of most theories regarding the onset of VR sickness. To test the hypothesis that the balance board as a control method would be less sickening than using joysticks, we designed a user study (N=32, 15 women) in which the participants drove a simulated differential drive robot in a virtual environment with either a Nintendo Wii Balance Board or joysticks. However, our pre-registered main hypotheses were not supported; the joystick did not cause any more VR sickness on the participants than the balance board, and the board proved to be statistically significantly more difficult to use, both subjectively and objectively. Analyzing the open-ended questions revealed these results to be likely connected, meaning that the difficulty of use seemed to affect sickness; even unlimited training time before the test did not make the use as easy as the familiar joystick. Thus, making the board easier to use is a key to enable its potential; we present a few possibilities towards this goal.

==> defs.tex <==


%% Use this to make index entries appear in the margin
%\usepackage{showidx}

%\usepackage[dvips,ps2pdf]{hyperref} 
%\usepackage{hyperref} 




%% Turn on/off math bold
\def\mbon{\mathversion{bold}}
\def\mboff{\mathversion{normal}}

%% Continuous-time definitions
\def\tf{{\phi}} %% State transition function

\def\queue{{Q}}

%% Nature actions
\def\nata{{\theta}}
\def\natas{{\Theta}} % All nature actions

\def\Xappr{{\hat{X}}} % Approximate state space
\def\Xfappr{{\tilde{X}}} % Approximate state space

%% Borrowed from Devin Balkcom and Matt Mason (ijrr 02 paper):
\newcommand{\FF}[0]{\ensuremath{\Uparrow}}
\newcommand{\BB}[0]{\ensuremath{\Downarrow}}
\newcommand{\LL}[0]{\ensuremath{\curvearrowleft}}
\newcommand{\RR}[0]{\ensuremath{\curvearrowright}}

\def\graph{{\cal G}}

\def\stages{{\cal K}}

\def\histy{{\tilde{y}}} %% History
\def\histu{{\tilde{u}}} %% History
\def\histv{{\tilde{v}}} %% History
\def\histx{{\tilde{x}}} %% History
\def\histz{{\tilde{z}}} %% History
\def\histp{{\tilde{p}}} %% History
\def\histe{{\tilde{e}}} %% History
\def\histtheta{{\tilde{\theta}}} %% History
\def\histyt{{\tilde{y}_t}} %% History
\def\histut{{\tilde{u}_t}} %% History
\def\histxt{{\tilde{x}_t}} %% History
\def\histthetat{{\tilde{\theta}_t}} %% History
\def\histpsit{{\tilde{\psi}_t}} %% History
\def\hspacey{{\tilde{Y}}} %% History
\def\hspaceu{{\tilde{U}}} %% History
\def\hspacex{{\tilde{X}}} %% History
\def\histpt{{\tilde{p}_t}} %% History
\def\histist{{\tilde \ist}}
\def\histq{{\tilde q}}
\def\histplan{{\tilde\plan}}

%% Information space notation
\def\ic{{\eta_0}} %% Initial condition
\def\ics{{{\cal I}_0}} %% Initial condition space
\def\ici{{\eta^i_0}} %% Initial condition
\def\icsi{{{\cal I}^i_0}} %% Initial condition space
\def\ist{{\eta}} %% Information state
\def\istder{{\eta_{der}}} %% Information state
\def\ifs{{\cal I}} %% An information space
\def\ifsder{{\cal I}_{der}} %% History information space
\def\ifsderp{{\cal I}'_{der}} %% History information space
\def\ifsest{{\cal I}_{est}} %% History information space
\def\ifshist{{\cal I}_{hist}} %% History information space
\def\ifsndet{{\cal I}_{ndet}} %% Nondeterministic information space
\def\ifsprob{{\cal I}_{prob}} %% Probabilistic information space
\def\ifsgauss{{\cal I}_{gauss}} %% Probabilistic information space
\def\ifsapp{{\cal I}_{app}} %% Probabilistic information space
\def\ifsmom{{\cal I}_{mom}} %% Probabilistic information space
\def\ifsk{{{\cal I}_k}} %% Native information space
\def\ifst{{{\cal I}_t}} %% Native information space
\def\imap{{\kappa}}
\def\imapndet{{\imap_{ndet}}}
\def\imapprob{{\imap_{prob}}}
\def\imapstage{{\imap_{stage}}}
\def\imapapp{{\imap_{app}}}
\def\imapmom{{\imap_{mom}}}
\def\imapgauss{{\imap_{mom}}}
\def\imapsf{{\imap_{sf}}}
\def\cifs{\ifs_c} %% Collapsed information space
\def\cist{\eta^c} %% Information space
\def\mifs{{\kappa}}
\def\imifs{{\Gamma^{-1}}}
\def\allp{{\Pi}} %% All plans
\def\allpc{{\Pi_\kappa}} %% All plans
\def\ite{{f_\ifs}} %% Information transition equation
\def\iteder{{f_\ifs}_{der}} %% Information transition equation
\def\hplan{{\cal H}} %% Information space
\def\difs{{\cal I}_\imap} %% Information space

\def\infX{{\vec{X}}}
\def\infx{{\vec{x}}}
\def\infU{{\vec{U}}}
\def\infu{{\vec{u}}}
\def\infTheta{{\vec{\Theta}}}
\def\inftheta{{\vec{\theta}}}
\def\inff{{\vec{f}}}
\def\infL{{\vec{L}}}
\def\infl{{\vec{l}}}


\def\Land{{\cal L}}

\def\ehat{\hat{e}}
\def\Ehat{\hat{E}}

\def\utility{{\cal U}}

% D^* definitions

\def\Gbest{{G_{best}}}
\def\Gcur{{G_{cur}}}
\def\Gvia{{G_{via}}}


%% This can be redef'ed later to be whatever we want for the robot
\def\A{{\cal A}}

%% Homeomorphism
\def\homeo{{ \;\cong\; }}

%%% The configuration space?
%\def\Q{{\cal Q}}

\def\choose#1#2{{(^{#1}_{#2})}}

\def\sgn{{\rm sgn}}
\def\sgnv{{\rm sgn}}

\def\pow{{\rm pow}}

\def\pdf{{p}}

%% closed chains
\def\Cclo{{{\cal C}_{clo}}}
\def\Cfea{{{\cal C}_{fea}}}


%% manip
\def\Csta{{{\cal C}_{sta}}}
\def\Cgr{{{\cal C}_{gr}}}
\def\Ctra{{{\cal C}_{tra}}}
\def\Cadm{{{\cal C}_{adm}}}
\def\Caobs{{{\cal C}^a_{obs}}}
\def\Cpobs{{{\cal C}^p_{obs}}}
\def\Capobs{{{\cal C}^{ap}_{obs}}}
\def\Xsta{{X_{sta}}}
\def\Xgr{{X_{gr}}}
\def\Xtra{{X_{tra}}}
\def\Ccon{{{\cal C}_{con}}}
\def\motcom{{\mu}}
\def\allmotcom{{\cal M}}


%%time var
\def\tva{{\tau}}
\def\tvb{{\sigma}}
\def\tvc{{\phi}}
\def\tvd{{g}}

%% multi
\def\multa{{\tau}}
\def\multb{{h}}
\def\cubesim{{\square}}

%% Conformation stuff
\def\confv{{q}}

%% General transformation
\def\gt{{h}}
\def\gti{{h^{-1}}}

%% Translation parameters
\def\xt{x_t}
\def\yt{y_t}
\def\zt{z_t}

%% Logical predicates
\def\lpred{\phi}
\def\qfpred{\phi}
\def\plpred{\alpha}
\def\quant{{\cal Q}}
\def\tarsk{\Phi}
\def\qftask{\phi}
\def\polys{{\cal F}} % Set of polynomials
\def\proot{{\beta}} % Polynomial root

%% Canny's method
\def\polyf{{\psi}}
\def\cmap{{h}}

%% C-space definitions
\def\C{{\cal C}}
\def\Cobs{{\cal C}_{obs}}
\def\Cfree{{\cal C}_{free}}
\def\CP{{P}}
\def\qinit{{q_{I}}}
\def\qgoal{{q_{G}}}
\def\qcur{{q_{cur}}}
\def\qnew{{q_{new}}}
\def\qiinit{{q^i_{I}}}
\def\qigoal{{q^i_{G}}}
\def\qoneinit{{q^1_{I}}}
\def\qonegoal{{q^1_{G}}}
\def\qminit{{q^m_{I}}}
\def\qmgoal{{q^m_{G}}}

\def\Xobs{{X_{obs}}}
\def\Xfree{{X_{free}}}
\def\Xcon{{X_{con}}}
\def\Xric{{X_{ric}}}
\def\xinit{{x_{I}}}
\def\xgoal{{x_{G}}}
\def\Xgoal{{X_{G}}}
\def\xcur{{x_{cur}}}
\def\xnew{{x_{new}}}

\def\B{{\cal B}}
\def\D{{\cal D}}
\def\I{{\cal I}}
\def\J{{\cal J}}
\def\K{{\cal K}}
\def\L{{\cal L}}
\def\M{{\cal M}}
\def\N{{\cal N}}
\def\O{{\cal O}}
\def\P{{\cal P}}
\def\U{{\cal U}}
\def\W{{\cal W}}
\def\X{{\cal X}}

\def\Ufree{{\U_{free}}}

% Mapping for a singular simplex
\def\sing{{\sigma}}

\def\x{{ x}}
\def\u{{ u}}

\def\Uf{{\vec U}}
\def\Vf{{\vec V}}
\def\Wf{{\vec W}}
\def\Zf{{\vec Z}}

% Complexes
\def\Comp{{\cal K}}
\def\Cell{C}
\def\Simp{\Delta}

% van der Corput sequence
\def\vdc{{\nu}}
% General sequence
\def\genseq{{\alpha}}

\def\Re{{\mathbb{R}}}
\def\Com{{\mathbb{C}}}
\def\Z{{\mathbb{Z}}}
\def\S{{\mathbb{S}}}
\def\H{{\mathbb{H}}}
\def\Q{{\mathbb{Q}}}
\def\Nat{{\mathbb{N}}}
\def\RP{{\mathbb{RP}}}
\def\F{{\mathbb{F}}}
\def\T{{\mathbb{T}}}
\def\One{{\bf 1_G}}
\def\Ra{{\mathbb{A}}}
\def\Vs{{V}}

\def\Fcal{{\cal F}}

\def\q{{q}}

%% Randomized strategy
\def\urand{{w}}

\def\qq1{{q_1}}
\def\qk{{q_k}}
\def\qi{{q_i}}
\def\qkp1{{q_{k+1}}}
\def\qKp1{{q_{F}}}
\def\qKi{{q_{K+1}}}
\def\qKp1{{q_{F}}}
\def\qi{{q_{F}}}
\def\qxq1{{q_1}}

\def\uu1{{u_1}}
\def\uk{{u_k}}
\def\uK{{u_K}}
\def\ui{{u_i}}
\def\xk{{x_k}}
\def\xi{{x_i}}
\def\xkp1{{x_{k+1}}}
\def\xKp1{{x_{F}}}
\def\xKi{{x_{F}}}
\def\xq1{{x_1}}
\def\ukp1{{u_{k+1}}}
\def\thetak{{\theta_k}}

% These are backward actions
\def\bwactset{{U^{-1}}}
\def\bwact{u^{-1}}
\def\bwf{{f^{-1}}}

\def\octg{G^*}        % Optimal cost to go
\def\octc{C^*}        % Optimal cost to come 
\def\eoctg{G^*}       % expected Optimal cost to go
\def\eoctc{C^*}       % expected Optimal cost to come 
\def\woctg{G^*}       % worst-case Optimal cost to go
\def\wctg{G}       % worst-case cost to go
\def\woctc{C^*}       % worst-case Optimal cost to come 
\def\ctg{{G}}         % Cost-to-go   -- not necessarily optimal
\def\ctgpl{{G_\plan}}         % Cost-to-go   -- not necessarily optimal
\def\wctgpl{{G_\plan}}         % Cost-to-go   -- not necessarily optimal
\def\ctc{{C}}         % Cost-to-come -- not necessarily optimal
\def\ectg{\hat{G}^*}  % Estimated cost-to-go (A-star)
\def\ctgs{{g}}         % Cost-to-go for use in sampling chapter -- conflict with G
\def\exctg{G}       % expected Optimal cost to go
\def\exctgpl{G_\plan}       % expected Optimal cost to go
\def\exctc{C}       % expected Optimal cost to come 
\def\eoj{J^*}
\def\eojpl{J_\plan}
\def\qval{Q^*}
\def\aqval{\hat{Q}^*}
\def\qvalpl{Q_\plan}
\def\eectg{\hat{G}_\plan}

\def\cmean{\bar{c}}

\def\topi{{/\sim}} % Topological identification
\def\xb{{x_b}}

\def\Polys{{\cal P}}
\def\Poly{{P}}

%% 2D phase space for trajectory planning
\def\tphase{{S}}

%% Game theory
\def\Pa{{{\rm P}_1}}
\def\Pb{{{\rm P}_2}}
\def\Pc{{{\rm P}_3}}
\def\Pli{{{\rm P}_i}}
\def\Pn{{{\rm P}_n}}
\def\upperv{\overline{L}^*}
\def\lowerv{\underline{L}^*}
\def\ecost{{\bar{L}}}
\def\uppervm{\overline{\cal L}^*}
\def\lowervm{\underline{\cal L}^*}
\def\gamev{L^*}
\def\gameva{{L^*_a}}
\def\gamevb{{L^*_b}}
\def\gamevm{{\cal L}^*}

%% Plan definitions
\def\plan{\pi}
\def\fplan{\pi} %% Feedback
\def\iplan{\pi}
\def\pplan{\sigma} %% Partial plan
\def\planset{{\Pi}}
\def\fplanset{{\Pi}}

\def\argmax{\operatornamewithlimits{argmax}}
\def\argmin{\operatornamewithlimits{argmin}}
\def\Pre{\operatorname{Pre}}
\def\Back{\operatorname{B}}
\def\SB{\operatorname{SB}}
\def\WB{\operatorname{WB}}
\def\Front{\operatorname{Front}}
\def\mymod{\operatorname{mod}}
\def\erf{\operatorname{erf}}
\def\hull{\operatorname{hull}}
\def\Front{\operatorname{Front}}
\def\atan2{\operatorname{atan2}}
\def\intfn{\operatorname{int}}
\def\dspan{\operatorname{span}}
\def\exp{\operatorname{exp}}
\def\adop{\operatorname{Ad}}
\def\clfn{\operatorname{cl}}
\def\Vor{\operatorname{Vor}}

\def\distr{{\triangle}}
\def\tdiff{{\Delta t}}
\def\lie{{\cal L}}
\def\phall{{\cal PH}}

\def\Cinfeq{{{\tilde C}^\infty}}

\def\truesp{\mbox{\sc{true }}}
\def\falsesp{\mbox{\sc{false }}}
\def\true{\mbox{\sc{true}}}
\def\false{\mbox{\sc{false}}}

\def\sccat{\mbox{\sc{cat}}}
\def\scdog{\mbox{\sc{dog}}}
\def\sctree{\mbox{\sc{tree}}}
\def\schouse{\mbox{\sc{house}}}

\def\qdot{{\dot q}}
\def\pdot{{\dot p}}
\def\qddot{{\ddot q}}
\def\qdddot{{q^{(3)}}}
\def\xdot{{\dot x}}
\def\xddot{{\ddot x}}
\def\yddot{{\ddot y}}
\def\ydot{{\dot y}}
\def\zdot{{\dot z}}
\def\xtdot{{{\dot x}_t}}
\def\ytdot{{{\dot y}_t}}
\def\thetadot{{\dot \theta}}
\def\thetaddot{{\ddot \theta}}
\def\adot{{\dot a}}
\def\bdot{{\dot b}}
\def\ceedot{{\dot c}}
\def\deedot{{\dot d}}
\def\fdot{{\dot f}}
\def\rdot{{\dot r}}
\def\sdot{{\dot s}}
\def\sddot{{\ddot s}}
\def\udot{{\dot u}}
\def\vdot{{\dot v}}
\def\wdot{{\dot w}}
\def\omegadot{{\dot \omega}}
\def\sigmadot{{\dot \omega}}
\def\phidot{{\dot \phi}}
\def\psidot{{\dot \psi}}
\def\alphadot{{\dot \alpha}}
\def\betadot{{\dot \beta}}
\def\gammadot{{\dot \gamma}}
\def\lambdadot{{\dot \lambda}}
\def\hdot{{\dot h}}
\def\gdot{{\dot g}}

\def\xtoq{{\kappa}}

\def\ustar{{u^*}}
\def\E{\operatorname{E}} %Expectation: $\E[X]$ (like \Pr)

\theoremstyle{plain}

%{\theorembodyfont{\rmfamily}\newtheorem{formulation}{Formulation}[chapter]}
%{\theorembodyfont{\rmfamily}\newtheorem{example}{Example}[chapter]}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Def}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{scenario}{Scenario}


\def\ds{\displaystyle\strut}
\def\idz{{\hspace{0.25in}}}

\def\disX{{\check X}}
\def\disx{{\check x}}
\def\disu{{\check u}}
\def\disU{{\check U}}
\def\disxgoal{{{\check x}_g}}
\def\disfplan{{\check \fplan}}
\def\disphi{{\check \phi}}

%% Dynamics
\def\force{{F}}
\def\moment{{N}}
\def\com{{p}} % Center of mass
\def\velcom{{\dot p}} % Center of mass
\def\acccom{{\ddot p}} % Center of mass
\def\mass{{m}}
\def\linmom{{D}} % Linear momentum
\def\angmom{{E}} % Angular momentum
\def\dens{{\sigma}}
\def\covfn{{\histx}} % Function for calculus of variations

\newcommand{\R}{{\mathcal R}}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}

\newcommand{\qed}{\hfill $\blacksquare$ \hfill \\}


